WiSM: Windowing Surrogate Model for Evaluation of Curvature-Constrained Tours with Dubins vehicle

Dubins tours represent a solution of the Dubins Traveling Salesman Problem (DTSP) that is a variant of the optimization routing problem to determine a curvature-constrained shortest path to visit a set of locations such that the path is feasible for Dubins vehicle, which moves only forward and has a limited turning radius. The DTSP combines the NP-hard combinatorial optimization to determine the optimal sequence of visits to the locations, as in the regular TSP, with the continuous optimization of the heading angles at the locations, where the optimal heading values depend on the sequence of visits and vice versa. We address the computationally challenging DTSP by fast evaluation of the sequence of visits by the proposed Windowing Surrogate Model (WiSM) which estimates the length of the optimal Dubins path connecting a sequence of locations in a Dubins tour. The estimation is sped up by a regression model trained using close to optimum solutions of small Dubins tours that are generalized for large-scale instances of the addressed DTSP utilizing the sliding window technique and a cache for already computed results. The reported results support that the proposed WiSM enables a fast convergence of a relatively simple evolutionary algorithm to high-quality solutions of the DTSP. We show that with an increasing number of locations, our algorithm scales significantly better than other state-of-the-art DTSP solvers.

==> src/removed.tex <==
% Filename: removed.tex
% Date:     2018/12/23 15:27
% Author:   Jan Faigl

% - introduction --------------------------------------------------------------
%which is otherwise computationally very demanding for a dense uniform sampling used in~\cite{manyam_dubins_2016}. 
% TODO a resolution complete sampling-based methods


%This heterogenous solution representation requires a black-box optimizer such as an Evolutionary Algorithm (EA).


% Although several DTSP solvers have been proposed in the literature~\cite{macharet18survey}, we consider a novel approach based on the recently published informed sampling of the possible heading angles~\cite{faigl17ecmr} in the solution of the DTSP with a given sequence of visits that is further called the \emph{Dubins Touring Problem} (DTP).
% The sampling is informed by the tight lower bound solution of the DTP~\cite{manyam_dubins_2016} that is computed using a closed-form solution of the Dubins Interval Problem which stands to determine the length of the shortest Dubins maneuver connecting two points but with specified angle interval for leaving and arrival angles of the vehicle~\cite{manyam2015shortest}.
% In~\cite{faigl17ecmr}, the lower bound enables finding a solution of the DTP close to optimum, i.e., with the relative optimality gap to the lower bound less than 1\%, in tens of seconds for problems with up to 100 locations, which is otherwise computationally very demanding for a dense uniform sampling used in~\cite{manyam_dubins_2016}. 


% On the other hand, both the approaches~\cite{manyam_dubins_2016,faigl17ecmr} use only a single sequence found as a solution of the Euclidean TSP without considering the minimum turning radius $\rho$ of the Dubins vehicle.
% Therefore, sampling-based approaches with very dense sampling and transformation of the problem to the Generalized TSP~\cite{oberlin2010today,obermeyer2012sampling} and evolutionary techniques~\cite{macharet12evolutionary,zhang2014memetic} may provide better solutions at the cost of very high computational requirements.
% In~\cite{faigl17ecmr}, it is reported that Memetic algorithm~\cite{zhang2014memetic} provides competitive solutions to the DTP-based approach for problems with up to 100 locations.
% However, the computational time is limited to one hour in comparison to the ten seconds of the DTP-based approach.



%Hence, the method might be understood as repeatedly running a \textit{decoupled} DTSP solver on EA-generated sequences \jd{(mozna vyhodit, ale libi se mi spojitost decoupled-joint)}.
%Note that while a solution representation in \textit{joint optimization} methods includes both location permutation and a vector of headings, the latter is not involved in our approach, significantly reducing the search-space for the EA. 

%\jd{(fakt to jinde nebylo pouzito?)} \pv{(PV: Jednou jsem nekde videl genetiku s AA, ale nemohu to najit, ale asi mozne vynechat)} 

%the theoretically sound TODO - PV: realy theoretically sound??

%\jd{(tyhle detaulni vysledky uz tu nejsou, ale asi ok)}. 

% The herein proposed \emph{Windowing Surrogate Model} (WiSM) leverages on the high-quality solution of the DTP~\cite{faigl17ecmr} that is employed in a relatively simple Evolutionary Algorithm (EA) for solving the DTSP.
% Even though the solution of the DTP by the informed sampling~\cite{faigl17ecmr} is significantly faster than the uniform sampling~\cite{manyam_dubins_2016}; it is still very demanding when employed in the EA where it is necessary to evaluate many candidate sequences.
% In~\cite{wang_global_2018}, the authors speed up expensive evaluation of the objective function using a surrogate model, and we similarly propose to evaluate candidate sequences using a surrogate model that is learned on small instances of the DTP.
% The model is further generalized by the proposed sliding window principle for arbitrarily long sequences to solve the DTSP.
% Thus, the WiSM enables to evaluate more candidate sequences within the given computational time, and thus improves convergence of the DTSP solution.


%- problem.tex ---------------------------------------------------------------
%include the closing trip connecting the last and the first location. 

%which can be found as a solution of the DTP.
%In this paper, we address the DTSP as an evaluation of possible sequences $\Sigma$, and we denote the cost of the solution for the particular sequence $\Sigma$ as $C(\Sigma)$. 

% - background-dtp.tex --------------------------------------------------------
%\jd{@Petr: hodne jsem to prorezal, zkontroluj prosim, ze to jeste furt dava smysl :) Nevyhodit jeste feasible vs. lower bound?}
% PV: podle me lower bound neni nutny, naprosto staci zminka o IRIS

% \begin{figure}[!htb]
%    \centering
%    \includegraphics[width=0.8\columnwidth]{fig/dtp_graph.pdf}
%    \caption{\label{fig:dtp_graph}
%    A graph representing discretized instance of the DTP where each layer corresponds to one location with $k$ heading samples.
%    }
% \end{figure}

% Having the states and their connections, a search graph shown in Fig.~\ref{fig:dtp_graph} can be created and the shortest path for the given sequence of $n$ locations and defined sampling $k$ can be found in $O(nk^3)$ by a forward search based on dynamic programming.

% \begin{figure}[!htb]
%    \subfloat[{\bf $C=19.8$}, $C_L=13.8$, \newline $N_k=7\cdot 32=224$, $\text{T}_\text{cpu}=128$~ms]{\includegraphics[height=2.7cm]{fig/dtp-uniform-32.pdf}}
%    \hfill
%    \subfloat[{\bf $C=14.4$}, $C_L=14.2$,\newline $N_k=128$,  $\text{T}_\text{cpu}=76$~ms]{\includegraphics[height=2.7cm]{fig/dtp-refine-128.pdf}}
%    \caption{Example of the DTP solution found by uniform (left) and informed sampling (right) using the total number of samples $N_k$.
%    The length of the solution is denoted $C$ and its lower bound is $C_L$.
%    \label{fig:dtp_example}
%    \vspace{-1em}
%    }
% \end{figure}

%A solution of the DTP can be improved by a more dense sampling of the heading angles; however, we can directly estimate the solution quality using a lower bound solution of the DTP that can be determined in the same way as a feasible solution. %using the graph in Fig.~\ref{fig:dtp_graph}. 
%The only change comes in using heading angle intervals instead of sole angles and computing the costs of the connecting edges as the closed-form solution of the Dubins Interval Problem~\cite{manyam2015shortest}.

%, see example in Fig.~\ref{fig:dtp_example}.

% The model is trained using a large dataset built upon high-quality solutions of small fixed-size DTP instances and the model is then generalized for arbitrarily long instances, see Section~\ref{sec:method}.



% - background-dtp.tex --------------------------------------------------------
%JF: not sure how much is goaoc2013bounded and D_4 relevant 
%\revise{A special case of the Dubins tour are DTP instances with the mutual distance between two consecutive locations in the sequence is longer than $4\rho$ and the instance is denoted $D_4$.
%The total tour length of Dubins tour of $D_4$ instances is a convex function and an optimal solution can be found using~\cite{goaoc2013bounded}; however, the number of possible combinations of the Dubins maneuver connecting two locations is still relatively high, and the authors bound it to $2^{n-2}$ for $n$ locations in the sequence.
%In general,} 

% - ea.tex --------------------------------------------------------------------


%In the case of \crossover, two parents are subsequently chosen.


% - method.tex ----------------------------------------------------------------

% Surrogate-Assisted Genetic Programming With Simplified Models for Automated Design of Dispatching Rules

%Even though the informed sampling-based method~\cite{faigl17ecmr} can approximate $C(\Sigma)$ with arbitrary precision (depending on the number of performed heading refinement iterations), it is impractically slow.
%Therefore, we propose the \textit{Windowing Surrogate Model} (WiSM) to replace the solution of the DTP with a surrogate function implemented using an artificial neural network for a specific part of the sequence, denoted as the sliding window.


%In particular, the WiSM approximates the IRIS DTP solver~\cite{faigl17ecmr} by a fast one-shot computation based mainly on highly-optimized matrix multiplications.


%The surrogate model can be efficiently learned for relatively short Dubins tours, and therefore, we propose sliding window principle to estimate the cost $C(\Sigma)$ of the DTP for longer sequences of the target locations $\mathcal{T}$.

% ------ Tady je dulezite, ze to neplati jen pro optimalni sekvenci. Plati to pro optimalni headings (pro libovolnou sekvenci). Myslim, ze to reviewer puvodne nepochopil, tak jsem to vic rozepsal. JD

%The whole Dubins tour of $n$ locations can be split into $n/w$ individual windows and the cost of the tour can be computed as a sum of the window costs.
%However, based on the preliminary evaluation of the cost estimation using such individual windows, a more precise estimation is provided for overlapping windows because each window is treated individually, and the total Dubins tour cost depends on the particular heading angles for the whole sequence.

%\todo{\jd{Predchozi vetu moc nechapu. Co je mysleno "preliminary evaluation"? Jsou to ty prvni experimenty, kdy jsme zkouseli neprekryvana okna? Vzhledem k tomu, ze na tomto miste jeste neni ani zminka o Open DTP, neni to pochopitelne.  Zde se jeste nebavime o "estimation", pokud sectu vsechny spravne $C^{*}_{w,i}(\Sigma)$ dostanu presnou hodnotu $C^*(\Sigma)$. Navic to plati jen pokud $w$ deli $n$. Myslim, ze to zbytecne zeslozituje text.}}
%\jf{nevidel bych to tak cerne, me prijde, ze to dava nahled proc to tak delema. Bude se to musi prepsat cele a rovnou pres overlapping a vubec to nerozvadet, nebo nejaka takova story.}

%Moreover, the overlapping window principle allows to address problem for which the number of locations $n$ is not divisible by the utilized window size $w$, i.e., $n \nmid w$.

%Now, if we consider the optimal solution of the $\overline{\text{DTP}}$ in (\ref{eq:cost}), it is expected the cost estimation converges to the optimal cost for an infinite window size
%\begin{equation}
%   \lim_{w \rightarrow \infty}\tilde{C}_w(\Sigma) \simeq C^*(\Sigma).
%\end{equation}

%\todo{\jd{Otazkou je, zda by nas z hlediska sekce Results nezajimalo i tvrzeni: $\tilde{C}_{w_1}(\Sigma) \leq \tilde{C}_{w_2}(\Sigma)$ pro $w_1 < w_2$.}}

% Tohle je trochu blabol, reaguju tim na vytku reviewera, ze na sliding window neni nic zvlastniho. Dulezite je, ze u WiSM mame nejakou teorii o tom, co ta vysledna agregovana hodnota predstavuje. To obecne neplati. Neco takoveho by tu melo rozhodne byt.

%Multiple neural network architectures can be considered that can follow a general architecture depicted in Fig.~\ref{fig:ann_approx}.

%This choice enables to compute the lower bound $\tilde{C}_w(\Sigma)$ end-to-end using a single network taking advantage of highly optimized tensor manipulation libraries, such as the TensorFlow~\cite{tensorflow2015-whitepaper}.
%The actual performance of the proposed model is reported in Section~\ref{sec:results}.

For any particular sequence $\Sigma$, let $C^*(\Sigma)$ be the cost of the optimal Dubins tour, i.e., the cost of the related DTP solution, and $Q^* = (q_1^*, \ldots, q^*_n)$ be the corresponding states with the optimal heading angles $\Theta^*$.
\ifnum\showfuture=1
\begin{framed}
   \todo{We should also prove that for $v < w$ the following holds: $C_v(\Sigma) \leq C_{w}(\Sigma)$.
   It is important for the window size experiments.}

\pv{
It can be easily shown that the estimation $C$ is non-decreasing when the number of Dubins maneuvers $w$ is doubled.
Thus:
\begin{equation}
C_{2w}(\Sigma) \geq C_{w}(\Sigma), \quad \forall w \in \mathbb{N}^+
\end{equation}
The proof is based on the idea that 
\begin{equation}
\overline{C}(\Sigma_i^w) + \overline{C}(\Sigma_{i+w}^w) \leq \overline{C}(\Sigma_i^{2w})
\end{equation}
Thus, we can assume that the estimation $C$ is non-decreasing with the window size.
However, it is not proven yet.
}

\todo{Having some guarantees (upper bound) would be great!}
\todo{Sum up levels at which any kind of approximation happens: Eq~\ref{eq:cost} and window size $w$, WiSM, EA. 
E.g., $\overline{DTP}1024$ is still an approximation of DTP.}

\todo{Add a graph showing $C(\Sigma)$ vs $C_w(\Sigma)$ for $n = 5$ and $w \in \{1, 2, \ldots, 25\}$.}
\end{framed}
\fi





%\todo{We are not exactly approximating $C_{\text{open}}$.
%Having something like $y^{(1)} < y^{(2)}$ for $C_{\text{open}}^{(1)} \leq C_{\text{open}}^{(2)}$ is sufficient ($y$ is monotonically increasing function of $C_{\text{open}}$?, see Wiki: \textit{monotonic transformation}.).
%Has to work with the tournament selection.
%Will this work with other selection operators too?}

%Besides, a naive approach to compute $C_w(\Sigma)$ would be to successively evaluate all $\overline{C}(\Sigma_1^w)$ through $\overline{C}(\Sigma_n^w)$ and then apply the weighted mean.
%However, we can take one step further by realizing that the whole operation can be seen as a one-dimensional convolution where the kernel of the size $w+1$ slides over $2n$ coordinates of all $n$ locations with the stride $s = 2$.

%\begin{figure}[!htb]
%   \centering
%   \includegraphics[width=\columnwidth,valign=c]{fig/cnn_approx.pdf}
%   \caption{
%      Convolutional neural network architecture for estimation of $\frac{w}{n}C_w(\Sigma)$.
%      The network accepts an arbitrary number of locations $n$.
%      The situation for $n = 8$ and window size $w = 3$ is shown here.
%      Dashed lines delimit the receptive areas of selected units (red cubes).
%      Only a sample of feature maps is visualized for convolutional layers one to three. 
%      \label{fig:cnn_approx}
%   }
%\end{figure}

%A straightforward convolutional extension to the original MLP architecture is depicted in Fig.~\ref{fig:ann_approx}.
%The convolutional network works with windows of the size $w$ represented by $2w$ coordinates.
%In most of the experimental evaluations, we use $w = 3$ which is also the case of the depicted architecture.
%While the network can process an arbitrary number of locations, for clarity, we present the case with $n = 8$.
%The individual layers are as follows.

%The input constitutes the coordinates for the locations $\sigma_1$ through $\sigma_n$ and also the wrapped copies $\sigma_{n+1}(= \sigma_{1})$ to $\sigma_{n+w+1}(= \sigma_{w+1})$ to cover all permutations $\Sigma_1^w$ through $\Sigma_n^w$.
%The input is processed with the 1D convolutional layer working with 128 kernels of the size $F = 2w$ and stride $s = 2$ (to align with two-dimensional coordinates of the input locations).
%Each of 128 feature maps constitutes $n$ units onto which ReLU non-linearity is applied.
%The next two 1D convolutional layers work with 128 kernels of the size $F= 1$ and stride $s = 1$ preserving the number of units per feature map.
%Both these layers use the ReLU as the activation function.
%The fourth convolutional layer reduces the number of feature maps to a single one.
%Each of its $n$ units corresponds to values $\overline{C}(\Sigma_1^w)$ through $\overline{C}(\Sigma_n^w)$.
%Finally, the last parameterless layer employs the Global Average Pooling~\cite{lin2013_nin} which gives $\frac{1}{n}\sum_{i=1}^{n}\overline{C}(\Sigma_i^w)$.
%Note that the normalization differs from (\ref{eq:cost}) by a factor $\frac{n}{w}$.
%This difference had no impact on DTSP optimization, and given that we treat $w$  as a constant mostly, it makes the network output independent on the number of targets rather than on the window size which we find more practical.

%This model is evaluated $n$ times for the successive tours of $w$ targets, and finally, the weighted sum is computed to give an estimation of the lower bound established in~(\ref{eq:cost}).
%Figure~\ref{fig:cnn_approx} shows the actual convolutional architecture we use in all the following experiments.

%\todo{CNNs are already used to process sequential data -- show a connection to our approach.}

%TODO add comments how the surrogate model is utilized in the EA
%Successively the fitness of each individual of the initial population is evaluated using the convolutional neural network model as described in the previous section.
%Note that in this particular step we exploit the parallel nature of data evaluating the whole population at once: we feed the network an input matrix of size $N\times 2n$ in a single step (\evaluatePopulation).

%Our approach is to use a global optimization method, specifically an evolutionary algorithm, to approximate the solution of Eq.~(\ref{eq:closed}).
%One possibility is to employ the DTP method~\cite{faigl17ecmr directly} which can approximate $C(\Sigma)$ with arbitrary precision.
%Unfortunately it turns out that when larger instances of the DTSP are in consideration, this straightforward approach is impractically slow. Hence we suggest replacing the DTP method with a surrogate function implemented using an Artificial Neural Network (WiSM).

%The problem with machine learning models such as WiSMs is that these models are mostly limited to a fixed sized input which in our case corresponds to a fixed number of targets $n$.
%One possible solution would be to base the surrogate model on a recurrent WiSM allowing us to process inputs of variable-length as sequences.

% - results.tex ---------------------------------------------------------------
%\subsection{Window Size\label{sec:sec:experiments_window_size}}

%The maximum number of samples in the IRIS method was $k_\text{max}=1024$, denoted as $\text{DTP}1024$.
%$k_\text{max}$ corresponds to the maximum heading angle resolution, and thus solutions found by the $\text{DTP}1024$ correspond to the uniform sampling with $k=1024$ samples, but with  significantly lower computational requirements because only a fraction of samples is utilized.


%The WiSM approximator was trained using Keras~\cite{chollet2015keras} with TensorFlow backend~\cite{tensorflow2015-whitepaper} running in Python~2.7\footnote{Sources of the WiSM would be available at \url{https://purl.org/comrob/wism}.}.

%The commonly used weight initialization schemata~\cite{glorot2010,he2015} assume standardized inputs and outputs. 
%Although these concerns are less critical for shallow architectures such as the one used here, we employed the standardization achieving slightly better results in training (data not shown here).
%Note that inputs were already standardized (drawn from ${\cal N}(0, 1)$), hence the standardization was applied to the output (cost) only.


Note that this experiment is computationally relatively cheaper than the preceding one, hence we decided for 10 fold increase in number of instances.

%The conclusion is that with an exception of impractically high densities (regarding the motivational surveillance missions), there is no need to maximize $w$, and $w=3$ is utilized.

%Taking only the shortest \SI{1}{s} limit into consideration (denoted $\text{WiSM}_1$ in the following), all three methods give results in very short times on mean: AA in \SI{1.2}{s}, baseline in \SI{1.3}{s} and $\text{WiSM}_1$ in \SI{2.6}{s}\footnote{Note that the additional time over the $1 s$ time limit is consumed by the call to the DTP.}

% - subsection ----------------------------------------------------------------
%\subsection{Evaluation Results in the Solution of the DTSP\label{sec:main_results}}
\ifnum\showfuture=1
\begin{framed}
\todo{There is still a question if to choose WiSM CPU or WiSM GPU for the following experiments. Now it is the WiSM GPU, but it obfuscates the results of ETSP initialization due to long TensorFlow initialization.}
\end{framed}
\fi


\begin{comment}
   \subsection{ETSP Initialization\label{sec:sec:experiments_etsp_init}}
   \todo \jd{Remove this section}
   In this section we check the importance of initializing the initial population by the ETSP. Fig.~\ref{fig:etsp_init} shows results for $f_{\text{ETSP}} = 0$ (no initialization) and $f_{\text{ETSP}} = 1$ (full initialization) for $n = 100$, $d = 1$.

\todo{Damn, now I realized, that the initialization is actually harmful (except for very small times $<$ 30 seconds) , everything is computed with the initialization. Should I rerun the experiments? I'll run initialization experiments for WiSM CPU.}

\begin{figure*}[t]
   \subfloat{\includegraphics[width=\columnwidth]{fig/limited_time_ETSP_init_100targets.pdf}}
   \hfill
   \subfloat{\includegraphics[width=\columnwidth]{fig/generations_ETSP_init_100targets.pdf}} 
   \caption{
     ETSP initialization influence on convergence for varying amounts of time (left) and generations (right). Results of ETSP initialized (WiSM $f_{\text{ETSP}} = 1$) and non-initialized (WiSM $f_{\text{ETSP}} = 0$) versions for $n = 100$ and $d = 1$. ETSP initialized DTP64 added for reference.
      \label{fig:etsp_init}
   }
\end{figure*}

\todo{This sections should show that ETSP initialization is good when extra short time limits are chosen. EA quickly compensates for the initialization.}

\todo{Point out, that the initialized DTP64 is doing slightly better (generation-wise, not time-wise) than both initialized and uninitialized which means that DTP64 is better approximation of DTP1024}
\end{comment}

For most following experiments we decided to work with density $d = 1$ as we believe that these instances reflect realistic tasks related to robot and/or UAV navigation.

%The window size $w = 1$ corresponds to the Euclidean distance and $C_1(\Sigma)$ degrades to the ETSP cost.
%using the procedure described above, i.e., each of the WiSM models fits $\overline{C}(\Sigma^{\bullet}_w)$ using its approximation $\overline{DTP}1024(\Sigma^{\bullet}_w)$ as a target. 



%\subsection{Discussion\label{sec:sec:experiments_discussion}}
%\jd{TODO: Paragraph on window size.}
%\todo \jd{Petr/Honza: please add some future work, i.e., 3D Dubins, Bezier curves..., I don't know the details.}
%\todo \jd{Paralelization.}

%We believe that similar approach may be applied for the with the limited budget.
%Moreover, the model should be extendible for touring problems in which the neighborhood areas are considered for the target locations.
%Such an extension would be possible based on recently proposed Generalized Dubins Interval Problem (GDIP)~\cite{vana2018gdip} which enables to solve DTSP with Neighborhoods (DTSPN) or DOP with Neighborhoods (DOPN)~\cite{penicka17icuas}.

%The actual number of training epochs never exceeded 300. 
%In case of DTSP, we trained three neural networks models and selected the best one according to the validation MSE, for each tested setup.
%The same WiSM was used for all $(n, d)$ pairs.

% - subsection ----------------------------------------------------------------
% the whole section on window size experiments was moved to a new file and commented out
%\input{src/results_window_size}


% \jd{WIRIS-EA (windowed, caching on) a IRIS-EA (full) only for cases when getting (cost) comparative results with other methods. For $n=500$ no result. For $d=0.1$ only WIRIS-EA\textsubscript{600}}


%\jd{Tady by melo byt jasne, ze $k_\text{max} = 64$ neni sampling koncoveho vyhodnoceni DTP, tam se pouziva $k_\text{max} = 1024$. Je to sem treba pripisovat?}

%The proposed WiSM exhibits interesting behavior for the window size $w=3$, which provides the best results.
%We identified four possible factors that might explain the behavior: 1. the distribution of the training data and the size of the dataset; 2. the selected WiSM architecture; 3. the training procedure; and 4. varying complexity of the learning problems for different values of $w$.
%Although we dedicated a detailed analysis to our future work, based on the reported results and also observations during the development, the proposed WiSM with $w=3$ provides a suitable trade-off between the provided solution quality and computational requirements.


%JF: SA_8 not clear Tcpu, it is 1.3 s or 1.2 s
%Cost-wise, $\text{WiSM}_{1}$ achieves a significantly better result $0.59$ than the other methods (AA: $1.32$, $\text{SA}_{4}$: $0.8$, $\text{SA}_{8}$: $0.7$) in \SI{1.3}{s}. 
%Average time the other methods need is \SI{0.06}{s} for AA, \SI{0.4}{s} for $\text{SA}_{4}$ and \SI{1.2}{s} for $\text{SA}_{8}$. 

%JF: not sure how much this is important here, it would be better for the DTSP computational survey 
%summary, our method achieved the lowest values of the mean normalized cost for all tested cases\footnote{With an exception of the smallest instance ($n = 25$) and high density ($d = 10$) where we observed SA to insignificantly outperform WiSM, although this happened for relatively long times greater than \SI{10}{s} (data not shown here).}. 

%JF: Again not clear why to describe LIO here, put it to the DTSP computational survey
%While LIO was always dominated by the other methods; for low $n = 25$ and medium-sized $n = 100$, AA was able to deliver the results in shortest time, albeit the normalized mean cost was always above $1$. 
%The ETSP baseline achieves reasonable results for the low-density instances. 

\jd{@JF: z ceho plyne ten index $r$ v $C_r$? Relative?}


==> src/results_window_size.tex <==
\subsection{Influence of the Window Size to Approximation of the WiSM\label{sec:sec:experiments_window_size}}

\begin{figure*}[t]
   \subfloat[Density $d=10.0$]{\includegraphics[width=0.48\textwidth]{{fig/window_size_d10.0_n100}.pdf}}
   \hfill
   \subfloat[Density $d=1.0$]{\includegraphics[width=0.48\textwidth]{{fig/window_size_d1.0_n100}.pdf}}

   \subfloat[Density $d=0.1$]{\includegraphics[width=0.48\textwidth]{{fig/window_size_d0.1_n100}.pdf}}
   \hfill
   \subfloat[WiSM evaluation on the DTSP benchmark data, $n=100$, $d=1$
   ]{
      \includegraphics[width=0.48\textwidth]{{fig/window_size_ann_d1.0_n100}.pdf}
      \label{fig:window_size_benchmark} 
   }
   \caption{
    Influence of the window size $w$ on the relative error $\epsilon_r$ of the approximation in the DTP instances with varying densities $d$ (a-c); and the normalized cost $C_r$ in the DTSP instances~(d). 
    The relative error $\epsilon_r$ is defined in (\ref{eq:relative_error}) and the normalized cost $C_r$ in (\ref{eq:normalized_cost}).
     \label{fig:window_size}
   }
\end{figure*}


The influence of the window size $w$ to the cost approximation error was studied for ten WiSMs that were trained for each value $w \in \{1, \ldots, 10\}$.
The models were then evaluated on a set of 100 random instances of $n = 100$ target locations with densities $d = \in \{10.0, 1.0, 0.1\}$ generated as described in Section~\ref{sec:experiments_setup}. 
In this case, the ordering of the locations $\Sigma$ is a random permutation.
The results are summarized in Fig.~\ref{fig:window_size}a--c, where the relative error 
\begin{equation}
\label{eq:relative_error}
\epsilon_r = \frac{C(\Sigma) - \tilde{C}_w(\Sigma)}{C(\Sigma)}
\end{equation}
is computed for two cases: (i) $\tilde{C}_w(\Sigma)$ computed according to (\ref{eq:cost}) with the WiSM approximation of $\overline{C}(\Sigma_{w,\bullet})$; and (ii) the same as the DTP approximation denoted $\overline{\text{DTP}}1024(\Sigma_{w,\bullet})$. 
The ground truth cost $C(\Sigma)$ is computed using $\text{DTP}1024(\Sigma)$.

All the error values are positive because of (\ref{eq:cost}), where $\tilde{C}_w(\Sigma)$ is a lower bound of $C(\Sigma)$.
The higher variance of the WiSM w.r.t. DTP is mostly caused by using ten different WiSMs per each value $w$, compared to a single call of the DTP method.
However, a single WiSM has also noticeably higher variance that we explain by the imperfect approximation caused by the training procedure and the selected architecture.
In the case of the DTP, the error monotonically decreases as $w$ increases for all densities, which is the expected behavior.

The choice of an appropriate window size has to be a trade-off between the precision and computational burden.
The observed behavior is different for the WiSM, except for the high density $d = 10$. 
Looking at the ``practical'' density $d = 1$, the error decrease stops at $w = 3$ and then stalls for the wider windows. 
This behavior is even more pronounced for ETSP-like instances having low density $d = 0.1$, where $w = 3$ represents a local minimum. 
This is further supported by the additional evaluation of $w\in\{2,\ldots, 9\}$ in the context of the proposed DTSP algorithm for $n = 100$, $d = 1$, see Fig.~\ref{fig:window_size_benchmark}. 
Thus, $w=3$ is utilized in the rest of the evaluation.

%An average computational time per single window for $w = 3$ was $\SI{1.9e-7}{s}$ for the caching version and $\SI{3.3e-6}{s}$ for the version without cache. 
An average computational time per a single window for $w = 3$ was $\SI{3.3}{\mu s}$ and $\SI{0.2}{\mu s}$ without and with the caching, respectively.
Note the report times were measured from evaluation of the whole population of $N =100$ individuals each representing $n = 100$ target locations in a single batch, i.e., the neural network was fed a $2(w+1) \times nM = 8 \times \num{10000}$ input matrices in each generation of \mbox{WiSM-EA}. 
